VidModEx: Interpretable and Efficient Black Box Model Extraction for High-Dimensional Spaces

In the domain of black-box model extraction, conventional methods reliant on soft labels or surrogate datasets struggle with scaling to high-dimensional input spaces and managing the complexity of an extensive array of interrelated classes. In this work, we present a novel approach that utilizes SHAP (SHapley Additive exPlanations) to enhance synthetic data generation. SHAP quantifies the individual contributions of each input feature towards the victim model's output, facilitating the optimization of an energy-based GAN towards a desirable output. This method significantly boosts performance, achieving a 16.45% increase in the accuracy of image classification models and extending to video classification models with an average improvement of 26.11% and a maximum of 33.36% on challenging datasets such as UCF11, UCF101, Kinetics 400, Kinetics 600, and Something-Something V2. We further demonstrate the effectiveness and practical utility of our method under various scenarios, including the availability of top-k prediction probabilities, top-k prediction labels, and top-1 labels.

==> sections/checklist.tex <==

\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The claim made in the abstract and introduction is justified by the empirical results from comparative analysis across different settings and datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitations have been discussed in \ref{sec:limitation} 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Theoretical Assumptions made in \ref{sec:prelim} is discussed thoroughly in \ref{A:shapproof}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: While experimentation details are described well to reproduce the code. Official code is submitted in the supplementary material, which also contains detailed instructions to compute the given results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: A detailed, easy-to-install package is given in the supplementary that has usage details and configurations used for this work. The datasets used in the work are standard and data-loader for the same is available in the code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: While the paper only presents an overview of hyperparameters across all experiments, there are discrepancies in each experiment based on the best performance they produce; hence, one can find the exact hyperparameter and optimizer in the configs present in the code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: With the high computational expense to extract individual model across different settings and datasets, running multiple runs or statistical analysis of each hyperparameter is very expensive in this context. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experimentation section \ref{sec:experiments} gives a detailed configuration of the Resources used and their execution time.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper complies with the NeurIPS code of ethics and continues to keep the author's identity anonymous. This is with discretion to my best knowledge.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: While there are no societal impacts, the impact on multiple service providers can be large, and it is at the discrepancy of the user. While also considering many of the service providers do have defence mechanisms, we have not evaluated our pipeline's effectiveness on these mechanisms as that is not an objective of our work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not pose any such risk as we only propose a pipeline.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We ensure that all datasets employed in our research are properly credited to their original creators. Each dataset utilized is selected based on its licensing explicitly allowing for research use, and these datasets are commonly recognized and widely used in the community. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have made the source code for this work available. Detailed instructions are included in the ReadMe.md file in the code repository, along with the relevant licensing files.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No Crowdsourcing or research with human subjects was done for this work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No research was done with human subjects. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> sections/waste.tex <==
\begin{theorem}[Hierarchical Approximation of SHAP Values]
Let $f$ be a model with input feature set $M$, partitioned into $k$ disjoint groups $G_1, G_2, \ldots, G_k$, such that $M = \bigcup_{i=1}^k G_i$ and $G_i \cap G_j = \emptyset$ for $i \neq j$. Let $\phi_i(f, x)$ denote the SHAP value for feature $i$ given input $x$.

Under the following properties:
\begin{enumerate}
    \item (Local Accuracy) $f(x) = g(x') = \phi_0 + \sum_i \phi_i x'_i$
    \item (Missingness) $x'_i = 0 \Rightarrow \phi_i = 0$
    \item (Consistency) If $f'_x(z') - f'_x(z' \setminus i) \geq f_x(z') - f_x(z' \setminus i)$ for all $z' \in \{0,1\}^M$, then $\phi_i(f', x) \geq \phi_i(f, x)$
    \item (Group Homogeneity) For any two features $i, j$ in the same group $G_k$, $\mathbb{E}[|\phi_i(f, x) - \phi_j(f, x)|] \leq \varepsilon$, where $\varepsilon$ is a small positive constant
\end{enumerate}

The hierarchical approximation of SHAP values for feature $i$ in group $G_k$ is given by:

\[\phi_i(f, x) \approx \frac{1}{|G_k|} \sum_t \phi_k^t(f)\]

where $\phi_k^t(f)$ is the Owen value for group $G_k$:

\[\phi_k^t(f) = \sum_{t: G_k \subseteq T \subseteq M \setminus \{i\}} \frac{|T \cap G_k|!(|G_k|-|T \cap G_k|-1)!}{|G_k|!} \cdot \frac{|T|!(|M|-|T|-1)!}{|M|!} \cdot [f(T \cup \{i\}) - f(T)]\]

This approximation becomes exact as $\varepsilon$ approaches 0 in Property 4.
\end{theorem}

\begin{proof}
We begin with the standard SHAP formula for feature $i$:

\[\phi_i(f, x) = \sum_{z' \subseteq x'} \frac{|z'|!(M - |z'| - 1)!}{M!} [f_x(z') - f_x(z' \setminus i)]\]

Given the partition of $M$ into groups $G_1, G_2, \ldots, G_k$, we can rewrite this as:

\[\phi_i(f, x) = \sum_k \sum_{z'_j \subseteq x'_j} \frac{|z'_j|!(|G_k| - |z'_j| - 1)!}{|G_k|!} [f_x(z'_j) - f_x(z'_j \setminus i)]\]

where $z'_j$ represents subsets within group $G_k$.

By Property 4 (Group Homogeneity), for any two features $i, j$ in $G_k$, we have:

\[\mathbb{E}[|\phi_i(f, x) - \phi_j(f, x)|] \leq \varepsilon\]

This implies that we can approximate the SHAP value of any feature in $G_k$ by the average SHAP value of the group:

\[\phi_i(f, x) \approx \frac{1}{|G_k|} \sum_{i \in G_k} \phi_i(f, x)\]

Now, we can express the group's contribution using Owen values:

\[\frac{1}{|G_k|} \sum_{i \in G_k} \phi_i(f, x) = \frac{1}{|G_k|} \sum_t \phi_k^t(f)\]

where $\phi_k^t(f)$ is the Owen value for group $G_k$ as defined in the theorem statement.

Properties 1-3 are preserved:
\begin{enumerate}
    \item Local Accuracy: The sum of all group contributions still equals $f(x) - \mathbb{E}[f(x)]$, preserving local accuracy.
    \item Missingness: If $x'_i = 0$, the entire group $G_k$ containing $i$ will have zero contribution, satisfying missingness.
    \item Consistency: If individual feature contributions are consistent, their group average will also be consistent.
\end{enumerate}

As $\varepsilon$ approaches 0, the approximation becomes exact because:

\[\lim_{\varepsilon \to 0} \mathbb{E}[|\phi_i(f, x) - \phi_j(f, x)|] = 0 \text{ for all } i, j \text{ in } G_k\]

This implies that all features within a group have identical SHAP values in the limit.

The hierarchical approximation reduces the computational complexity from $O(2^M)$ to $O(2^k)$, where $k$ is the number of groups and $k \ll M$, providing a more efficient method for estimating feature importance in high-dimensional models.

Therefore, we have proven that the hierarchical approximation of SHAP values using partition explainer satisfies the required properties, converges to the true SHAP values as group homogeneity increases, and provides a computationally efficient method for estimating feature importance in high-dimensional models.
\end{proof}




\subsection{Proof of Shapley values and owen values}\label{A:shapproof}

Given the complex interactions among features in high-dimensional models, it is crucial to attribute the model's prediction accurately back to the contributing features. The additive feature attribution methods provide a framework, with Shapley values offering a theoretically sound approach under certain axiomatic properties. Building upon the foundational Theorem 1, which establishes the uniqueness of Shapley values under properties of local accuracy, missingness, and consistency, we propose a new theorem for hierarchical Shapley values derived from Owen values.


\subsection*{Theorem 2: Hierarchical Shapley Values from Owen Values}
Under the framework established by Theorem 1 and the hierarchical structure of the input space \( M \), where \( M \) is divided into \( k \) groups such that \( M = \bigcup_{i=1}^k G_i \) with \( G_i \cap G_j = \emptyset \) for all \( i \neq j \), the Shapley values derived from Owen values can uniquely be determined by the following approach:

\subsubsection*{Definition}
Let \( f \) be the targeted black-box model mapping input vectors to outputs, and let \( f(S) \) denote the output of the model when only the features in set \( S \subseteq M \) are active. The Owen value for feature \( i \) considering the hierarchical decomposition is given by Eq.\ref{eq:grouppartitiondef}. Where \( T \) as any subset of \( M \) that includes the group \( G_i \) but excludes a specific feature \( i \). Hence, \( T \) ranges over all such subsets where \( G_i \subseteq T \subseteq M \setminus \{i\} \).



\begin{equation}
\phi_i^T(f) = \sum_{T: G_i \subseteq T \subseteq M \setminus \{i\}} \frac{|T \cap G_i|!(|G_i|-|T \cap G_i|-1)!}{|G_i|!} \cdot \frac{|T|!(|M|-|T|-1)!}{|M|!} \cdot [f(T \cup \{i\}) - f(T)]
\label{eq:grouppartitiondef}
\end{equation}


\subsubsection*{Hierarchical Shapley Value Computation}
The hierarchical Shapley value for each feature \( j \) in the input space \( M \), which complies with the properties of local accuracy, missingness, and consistency as per Theorem 1, is computed as:
\begin{equation}
\phi_j(f, x) = \sum_{z_0 \subseteq x_0} \frac{|z_0|!(|M| - |z_0| - 1)!}{|M|!} [f_x(z_0 \cup \{j\}) - f_x(z_0 \setminus \{j\})]
\end{equation}
where \( x_0 \) represents the simplified input mapping \( hx \), and \( z_0 \subseteq x_0 \) represents all vectors \( z_0 \) where the non-zero entries are a subset of the non-zero entries in \( x_0 \).

\section*{Estimating Individual Feature Contributions from Group Contributions}

In many practical applications, particularly within the field of machine learning interpretability, it is often computationally infeasible or analytically complex to directly compute the Shapley values for each individual feature within a large dataset or a complex model. To address this challenge, we employ a method that approximates the contribution of individual features based on the aggregated contributions of their respective groups.

\subsection*{Hierarchical Decomposition}

Consider a model \( f \) mapping input vectors from a feature set \( M \) to outputs. The feature set \( M \) is divided into disjoint groups \( G_i \), each containing features that share certain characteristics or are expected to interact similarly within the model.

\subsection*{Group and Individual Feature Contributions}

The contribution of an entire group \( G_i \) to the model's output is calculated as a block, and then this contribution is distributed evenly among the features within the group. This approach assumes homogeneity within the group regarding their influence on the model's output.

\subsubsection*{Definition and Calculation}

Let \( f(S) \) denote the output of the model when only the features in set \( S \subseteq M \) are active. For a specific feature \( j \) within the group \( G_i \), the contribution is approximated by:
\begin{equation}
\phi_j(f, x \cup \{j\}) = \frac{\phi_i(f, T \cup G_i)}{|G_i|}
\end{equation}
where \( T \) is any subset of \( M \) that includes the group \( G_i \) but excludes the specific feature \( j \). This formula implies that \( T \) ranges over all such subsets where \( G_i \subseteq T \subseteq M \setminus \{j\} \).

This approximation distributes the estimated total contribution of the group \( G_i \) equally among its constituent features, reflecting the average effect of including each feature in the group on the model's output.

\somnath{ello}

\section{Derivation of Hierarchical Shapley Values from Owen Values}\label{A:shapcompute1}

\subsection{Theorem on Hierarchical Shapley Values}\label{A:shapproof1}

\textbf{Definition: Group-Based Shapley Values.} Consider a model \( f \) mapping input vectors from a feature set \( M \) divided into disjoint groups \( G_i \), where \( M = \bigcup_{i=1}^k G_i \) and \( G_i \cap G_j = \emptyset \) for all \( i \neq j \). The Owen value for a feature \( i \) within group \( G_i \) is defined by the equation:
\begin{equation}
\phi_i^T(f) = \sum_{T: G_i \subseteq T \subseteq M \setminus \{i\}} \frac{|T \cap G_i|!(|G_i|-|T \cap G_i|-1)!}{|G_i|!} \cdot \frac{|T|!(|M|-|T|-1)!}{|M|!} \cdot [f(T \cup \{i\}) - f(T)]
\label{eq:grouppartitiondef1}
\end{equation}

\textbf{Theorem: Hierarchical Shapley Value Computation.} Under the framework where \( M \) is divided into \( k \) groups and using the definition above, the Shapley value for each feature \( j \) in group \( G_i \) is computed by reducing the group Owen value to individual feature contributions:
\begin{equation}
\phi_j(f, x) = \frac{1}{|G_i|} \sum_{T: G_i \subseteq T \subseteq M \setminus \{j\}} \phi_i^T(f)
\label{eq:hierachicalShapley}
\end{equation}
where \( T \) is any subset of \( M \) including the group \( G_i \) but excluding feature \( j \), and \( |G_i| \) is the number of features in group \( G_i \).

\textbf{Approximation Concerns:} This method assumes that each feature within \( G_i \) contributes equally to the output of \( f \), potentially overlooking the unique impact of individual features within the group. This approximation simplifies the computation but may lead to inaccuracies in feature importance attribution for models where intra-group feature interactions are significant.
% \subsection*{Practical Implications and Assumptions}

% This method leverages the homogeneity assumption within groups, which may not always hold, especially if certain features disproportionately influence the model. However, it offers a significant reduction in computational complexity and can be particularly effective in hierarchical or layered models where features are naturally segmented into groups.

% \subsection*{Conclusion}

% By using group-based contributions to approximate individual feature impacts, we provide a feasible and efficient way to interpret complex models, making the explanation of model behavior accessible and manageable for stakeholders. This approach is a practical compromise between computational efficiency and interpretive granularity.



\section*{Hierarchical Decomposition of Contributions in Cooperative Game Theory Applied to Machine Learning Models}

In the analysis of machine learning models, particularly those considered as black-boxes, understanding the contribution of individual features is crucial. This can be analogously studied through concepts derived from cooperative game theory, notably the Shapley values and Owen values. In this context, we redefine the classical game-theoretic approach to accommodate a model's feature space.

\subsection*{Definitions and Notation}
Let \( M \) be the set of all features in the input space of a black-box model \( f \), which maps input vectors to an output space. The set \( M \) consists of \( k \) groups such that \( M = \bigcup_{i=1}^k G_i \) and \( G_i \cap G_j = \emptyset \) for all \( i \neq j \). Each group \( G_i \) may represent a subset of features that interact or are related in a particular way, perhaps due to their similar nature or collective impact on the model's output.

The function \( f \) is a characteristic function in this cooperative game, assigning a real number to each subset of features, indicative of the output's dependency on those features.

\subsection*{Hierarchical Contribution Calculation}
The contribution of each feature, and by extension each group of features, is assessed by the following hierarchical decomposition:

\subsubsection*{Group-Level Contribution}
The contribution of a group \( G_i \) to the overall model output is computed by considering the group as a single entity within the larger set:
\begin{equation}
\phi_{G_i}(f) = \sum_{T \subseteq M \setminus G_i} \frac{|T|!(|M|-|T|-|G_i|)!}{|M|!} \cdot [f(T \cup G_i) - f(T)]
\end{equation}
Here, \( T \) represents a coalition of groups excluding \( G_i \).

\subsubsection*{Individual Feature Contribution Within Groups}
Within each group \( G_i \), the contribution of an individual feature \( i \) is calculated using the Shapley value formula adapted for the subgroup:
\begin{equation}
\phi_i^{G_i}(f) = \sum_{S \subseteq G_i \setminus \{i\}} \frac{|S|!(|G_i|-|S|-1)!}{|G_i|!} \cdot [f(S \cup \{i\}) - f(S)]
\end{equation}

\subsection*{Integration of Contributions}
The Owen value for a feature \( i \), reflecting both intra-group dynamics and inter-group interactions, is given by:
\begin{equation}
\phi_i^O(f) = \sum_{T: G_i \subseteq T \subseteq M \setminus \{i\}} \frac{|T \cap G_i|!(|G_i|-|T \cap G_i|-1)!}{|G_i|!} \frac{|T|!(|M|-|T|-1)!}{|M|!} \cdot [f(T \cup \{i\}) - f(T)]
\end{equation}


This hierarchical approach to computing contributions of features provides a nuanced view that is particularly useful for interpreting the behavior of complex models in machine learning. By treating the feature space as a cooperative game, we can apply game-theoretical insights to understand how individual and groups of features influence model predictions, providing a bridge between machine learning interpretability and cooperative game theory.



\begin{theorem}[Hierarchical Approximation of SHAP Values]
Let $f$ be a model with input feature set $M$, partitioned into $k$ disjoint groups $G_1, G_2, \ldots, G_k$, such that $M = \bigcup_{i=1}^k G_i$ and $G_i \cap G_j = \emptyset$ for $i \neq j$. Let $\phi_i(f, x)$ denote the SHAP value for feature $i$ given input $x$.

Under the following properties:
\begin{enumerate}
    \item (Local Accuracy) $f(x) = g(x') = \phi_0 + \sum_i \phi_i x'_i$
    \item (Missingness) $x'_i = 0 \Rightarrow \phi_i = 0$
    \item (Consistency) If $f'_x(T \cup \{i\}) - f'_x(T) \geq f_x(T \cup \{i\}) - f_x(T)$ for all $T \subseteq M \setminus \{i\}$, then $\phi_i(f', x) \geq \phi_i(f, x)$
    \item (Group Homogeneity) For any two features $i, j$ in the same group $G_k$, $\mathbb{E}[|\phi_i(f, x) - \phi_j(f, x)|] \leq \varepsilon(|G_k|)$, where $\varepsilon(|G_k|)$ is a small positive constant that decreases as $|G_k|$ decreases
\end{enumerate}

The hierarchical approximation of SHAP values for feature $i$ in group $G_k$ is given by:

\[\phi_i(f, x) \approx \frac{1}{|G_k|} \sum_t \phi_k^t(f)\]

where $\phi_k^t(f)$ is the Owen value for group $G_k$:

\[\phi_k^t(f) = \sum_{T: G_k \subseteq T \subseteq M \setminus \{i\}} \frac{|T \cap G_k|!(|G_k|-|T \cap G_k|-1)!}{|G_k|!} \cdot \frac{|T|!(|M|-|T|-1)!}{|M|!} \cdot [f(T \cup \{i\}) - f(T)]\]

This approximation improves as $\varepsilon(|G_k|)$ decreases with smaller group sizes. However, the optimal group size is determined by balancing approximation accuracy with computational efficiency, constrained by a maximum number of allowed function evaluations $\text{max\_eval}$.
\end{theorem}

\begin{proof}
We begin with the standard SHAP formula for feature $i$:

\[\phi_i(f, x) = \sum_{T \subseteq M \setminus \{i\}} \frac{|T|!(|M| - |T| - 1)!}{|M|!} [f(T \cup \{i\}) - f(T)]\]

Given the partition of $M$ into groups $G_1, G_2, \ldots, G_k$, we can rewrite this as:

\[\phi_i(f, x) = \sum_k \sum_{T_k: G_k \subseteq T \subseteq M \setminus \{i\}} \frac{|T_k \cap G_k|!(|G_k|-|T_k \cap G_k|-1)!}{|G_k|!} \cdot \frac{|T|!(|M|-|T|-1)!}{|M|!} [f(T \cup \{i\}) - f(T)]\]

where $T_k$ represents subsets containing group $G_k$.

By Property 4 (Group Homogeneity), for any two features $i, j$ in $G_k$:

\[\mathbb{E}[|\phi_i(f, x) - \phi_j(f, x)|] \leq \varepsilon(|G_k|)\]

This allows for the approximation of the SHAP value of any feature in $G_k$ by the average SHAP value of the group:

\[\phi_i(f, x) \approx \frac{1}{|G_k|} \sum_{i \in G_k} \phi_i(f, x)\]

The group's contribution can be expressed using Owen values:

\[\frac{1}{|G_k|} \sum_{i \in G_k} \phi_i(f, x) = \frac{1}{|G_k|} \sum_t \phi_k^t(f)\]

where $\phi_k^t(f)$ is the Owen value for group $G_k$ as defined in the theorem statement.

Properties 1-3 are preserved in this approximation:
\begin{enumerate}
    \item Local Accuracy: The sum of all group contributions equals $f(x) - \mathbb{E}[f(x)]$, preserving local accuracy.
    \item Missingness: If $x'_i = 0$, the entire group $G_k$ containing $i$ will have zero contribution, satisfying missingness.
    \item Consistency: Group average contributions maintain consistency if individual feature contributions are consistent.
\end{enumerate}

As $\varepsilon(|G_k|)$ approaches 0 with decreasing group size:

\[\lim_{|G_k| \to 1} \varepsilon(|G_k|) = 0\]

implying that all features within a group have identical SHAP values in the limit, and the approximation becomes exact as group sizes approach 1.

The hierarchical approximation reduces the computational complexity from $O(2^M)$ to $O(2^k)$, where $k$ is the number of groups and $k \ll M$. To balance accuracy and computational efficiency, an optimal group size is determined by:

\[\text{optimal\_group\_size} = \arg \min_{|G_k|} \varepsilon(|G_k|) \text{ subject to } 2^k \leq \text{max\_eval}\]

where $\text{max\_eval}$ is the maximum number of allowed function evaluations.

This optimization ensures the best possible approximation within the given computational constraints. Therefore, the hierarchical approximation of SHAP values using partition explainer satisfies the required properties, converges to the true SHAP values as group sizes decrease, and provides a computationally efficient method for estimating feature importance in high-dimensional models, with the flexibility to balance accuracy and efficiency based on available computational resources.
\end{proof}
